Which Syntactic Capabilities Are Statistically Learned by Masked Language Models for Code?

This paper discusses the limitations of evaluating Masked Language Models (MLMs) in code completion tasks. We highlight that relying on accuracy-based measurements may lead to an overestimation of models' capabilities by neglecting the syntax rules of programming languages. To address these issues, we introduce a technique called SyntaxEval in which Syntactic Capabilities are used to enhance the evaluation of MLMs. SyntaxEval automates the process of masking elements in the model input based on their Abstract Syntax Trees (ASTs). We conducted a case study on two popular MLMs using data from GitHub repositories. Our results showed negative causal effects between the node types and MLMs' accuracy. We conclude that MLMs under study fail to predict some syntactic capabilities.

==> tabs/results_global.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[]

\centering
\caption{\syntaxeval Global Performance Results of $M_1$ and $M_2$ by Masking Control $T_0$ \& Treatment $T_1$}
\label{tab:global_results}
\vspace{-0.5em}
\scalebox{0.7}{

\setlength{\tabcolsep}{4pt} 

\begin{tabular}{cllll}
\hline
\textbf{Model}               & \textbf{Performance Metric $Y$}                    & \multicolumn{1}{c}{\textbf{Group}} & \multicolumn{1}{c}{\textit{\textbf{$avg \pm std$}}} & \multicolumn{1}{c}{\textit{\textbf{Median}}} \\ \hline
\multirow{6}{*}{\textbf{M1}} & \multirow{2}{*}{\textbf{Jaccard}}       & $T_1$                          & 0.78 $\pm$ 0.21                                      & 0.83                                         \\
                             &                                         & $T_0$                            & 0.88 $\pm$ 0.17                                      & 0.95                                         \\
                             & \multirow{2}{*}{\textbf{Levenshtein}}   &  $T_1$                          & 0.78 $\pm$ 0.22                                      & 0.84                                         \\
                             &                                         & $T_0$                            & 0.87 $\pm$ 0.16                                      & 0.95                                         \\
                             & \multirow{2}{*}{\textbf{Sorensen-Dice}} &  $T_1$                          & 0.85 $\pm$ 0.17                                      & 0.91                                         \\
                             &                                         & $T_0$                            & 0.92 $\pm$ 0.1                                       & 0.97                                         \\ \hline
\multirow{6}{*}{\textbf{M2}} & \multirow{2}{*}{\textbf{Jaccard}}       &  $T_1$                          & 0.76 $\pm$ 0.21                                      & 0.81                                         \\
                             &                                         & $T_0$                            & 0.84 $\pm$ 0.16                                      & 0.88                                         \\
                             & \multirow{2}{*}{\textbf{Levenshtein}}   &  $T_1$                          & 0.76 $\pm$ 0.21                                      & 0.81                                         \\
                             &                                         & $T_0$                            & 0.83 $\pm$ 0.17                                      & 0.88                                         \\
                             & \multirow{2}{*}{\textbf{Sorensen-Dice}} &  $T_1$                          & 0.84 $\pm$ 0.17                                      & 0.89                                         \\
                             &                                         & $T_0$                            & 0.89 $\pm$ 0.12                                      & 0.93                                         \\ \hline
\end{tabular}


} % % End Scalebox
\vspace{-1em}
\end{table}


==> text/6_limitations.tex <==
\section{Limitations}
\label{sec:limitations}

A thread to validity is that the masking of tokens may remove importing information from the context in the input for the model to perform accurate predictions, However the similarity scores revealed that still the model are able to predict the masked elements better than random. Despite this fact, causal effects are consistent since the size of the samples, the number of AST nodes and all confounders in $Z$ were controlled. Future research should address this problem by formulating different treatment strategies. 
